The Aligned-Coordinated Geographical Routing for Multihop Wireless Networks

The stateless, low overhead and distributed nature of the Geographic routing protocols attract a lot of research attentions recently. Since the geographic routing would face void problems, leading to complementary routing such as perimeter routing which degrades the performance of geographic routing, most research works are focus on optimizing this complementary part of geographic routing to improve it. The greedy forwarding part of geographic routing provides an optimal routing performance in terms of path stretch. If the geographic routing could adapt the greedy forwarding more, its performance would be enhanced much more than to optimize the complementary routing such as perimeter routings. Our work is the first time to do so. The aligned physical coordinate is used to do the greedy forwarding routing decision which would lead more greedy forwarding. We evaluate our design to most geographic routing protocols, showing it helps much and maintain the stateless nature of geographic routing.

==> intuition.tex <==
\section{Connection Sensitive Coordinates}

